Stein Variational Message Passing for Continuous Graphical Models

We propose a novel distributed inference algorithm for continuous graphical models, by extending Stein variational gradient descent (SVGD) to leverage the Markov dependency structure of the distribution of interest. Our approach combines SVGD with a set of structured local kernel functions defined on the Markov blanket of each node, which alleviates the curse of high dimensionality and simultaneously yields a distributed algorithm for decentralized inference tasks. We justify our method with theoretical analysis and show that the use of local kernels can be viewed as a new type of localized approximation that matches the target distribution on the conditional distributions of each node over its Markov blanket. Our empirical results show that our method outperforms a variety of baselines including standard MCMC and particle message passing methods.

==> tex/algorithm.tex <==
%\section{Our approach}

%The random variables are assumed to take values on a continuous space.
% Graphical models have a form of
% $$
% \log p(x) = \sum_{\alpha \in \C} \phi(x_\alpha),
% $$
% where $C$ is the set of graph cliques of the graphical model,
% and correspondingly the derivative of $\log p$ also have a nice total structure,
% $$
% \partial_{x_i} \log p(x) = \sum_{\alpha \in \C} \partial_{x_i} \phi(x_\alpha),
% $$
% where $x_i$ is the $i^{th}$ dimension of $x$. Recall that the SVGD update is,
% $$
% x \leftarrow x + \epsilon \phi(x)
% $$
% with
% $$
% \phi(x) = \frac{1}{n} \sum_{\ell=1}^n [\nabla \log p(x^\ell)K(x, x^\ell) + \nabla_{x^\ell} K(x,x^\ell)].
% $$






==> tex/converge.tex <==
% \section{TODOs}
\subsection{Discussions on the Convergence Property}
%\red{appendix?}

In this section, we discuss convergence properties of our approach.
Given a set of particles $\{x^{\ell, s}\}_{\ell=1}^n$
at the $s$-th iteration, 
where $n$ is the number of particles
and its distribution $q_s^n$ is unknown to us;
% in this case the distributional information of the particles is best
% represented by 
we denote its empirical distribution as $\hat{q}_{s}^n$.
In this section, we show that when $n \rightarrow \infty, s \rightarrow \infty$,
the empirical marginal distributions $\hat{q}_{s}^n(x_{\C_i})$ weakly converge to the
target marginal distributions $p(x_{\C_i}), \forall i \in [d]$ in the sense that we have
$\E_{\hat{q}_s^n(x_{\C_i})}[h] \rightarrow \E_{p(x_{\C_i})}[h]$ for all bounded, continuous test functions $h$.
% The empirical measure of $\{x_i^\ell\}_{\ell=1}^n$ at the $\ell$-th
% iteration of SVGD particles convergence to
% the target probability measure as $n \rightarrow \infty$ and
% $\ell \rightarrow \infty$.
% in the sense that we have $\E_{\u_n}[h] \rightarrow \E_{\nu_p}$

Our results are based on the theoretical analysis on SVGD in \citet{2017arXiv170407520L}.
We first show that for a fixed iteration $s$,
% when the number of particles $n \rightarrow \infty$ at a fixed iteration step $s$,
% \red{some conclusions here.}
the empirical distribution $\hat{q}_s^n$ will weakly converge to 
the limit distribution $q_s^\infty$ as the number of particles $n \rightarrow \infty$.
Here, our proof is based on the $L1-$Wasserstein distance 
rather than the bounded Lipschitz metric applied in \citet{2017arXiv170407520L}.
Without the bounded constrains on functions,
the $L1-$Wasserstein distance can be applied to a wider range of functions, defined as bellows.
% Then we show the iterative transformations in \eqref{equ:gsvgd}
% of our algorithm monotonically decreases the KL divergence between $q_s^\infty$ and the target distribution $p$.
% Note that the updates in original SVGD is defined in the same RKHS
% with the associated kernel defined over all coordinates.
% However, we use structured kernels $k_i$ for different coordinates $i$ specified by $\N_i$,
% which leads to a Stein discrepancy with graphical structures whose relationship with KL divergence measuring the whole coordinates is less straightforward.
% Still, we can show that under structured kernels, the decrease of KL divergence is bounded by the Stein discrepancy with graphical structures.


% For the first proof of weak convergence, 
% we adopt the $L1-$Wasserstein distance. 
% % to show the weak convergences of empirical distributions
% Without the bounded constrains on functions, the $L1-$Wasserstein distance can be applied to a wider range of functions
% than the bounded Lipschitz metric applied in \citet{2017arXiv170407520L}.
% Moreover, 
% the updates in SVGD is defined in the same RKHS
% with the associated kernel defined over all coordinates.
% However,
% we use structured kernels $k_i$ for different coordinates $i$ specified by $\N_i$,
% which leads to a Stein discrepancy with graphical structures whose relationship with KL divergence measuring the whole coordinates is less straightforward.
% Still, we can show that under structured kernels, the decrease of KL divergence is bounded by the Stein discrepancy with graphical structures.


% The convergence properties of our graphical SVGD with graphical structured kernels
% that of SVGD has been well discussed in \citep{2017arXiv170407520L},
% are immediate results from 
% Our results in based on \citet{2017arXiv170407520L},
% To make the content self-contained, we detailed our
% results as belows.

% Assume the empirical distribution $\hat{q}_s^n$ at the $s$-th iteration 
% is obtained by recursively applying
% map $\Phi_p$ starting from the initial empirical distribution $\hat{q}_0^n$,
% where 
% We first show that for a fixed iteration $s$,
% % when the number of particles $n \rightarrow \infty$ at a fixed iteration step $s$,
% % \red{some conclusions here.}
% the empirical distribution $\hat{q}_s^n$ will weakly converge to 
% the limit distribution $q_s^\infty$ as $n \rightarrow \infty$.

% Our derivations are based on the $L1-$Wasserstein distance of probability distributions
% which is defined as bellows,

% We will first introduce definition of Wasserstein distance to show large sample limit of empirical distributions. 
% Then a monotonically limiting behavior of our graphical SVGD dynamics is shown.
% \red{TODO: correct symbols}



% \begin{mydef}
% Let $\mathscr{P}(\X)$ denote the collection of all probability distributions on metric space $\X$ with finite mean.  
% Then the
% % Kantorovich or 
% $L_1-$Wasserstein distance between two probability distributions $q$ and $q'$ 
% in $\mathscr{P}(\X)$ is defined as
\begin{equation}
\mathcal{W}_1(q,q') := \inf\limits_{\gamma \in \Gamma(q,q')} \int|x-x^\prime|d\gamma(x,x^\prime),
\end{equation}
where $\Gamma(q,q')$
% $ \subseteq \mathscr{P}(\X \times \X)$ 
is the family of joint distributions on $\X \times \X$ with marginal distributions being $q$ and $q'$ on the first and second factors respectively.
% \end{mydef}
Then we characterize the weak convergence of empirical distribution with the $L1-$Wasserstein distance as follow.

% Define a map $\Phi_p: \mu \mapsto T_{\mu,p} \mu$ characterizing graphical SVGD dynamics, where $T_{\mu,p}$ is the update rule of particles with distribution $\mu$, that is each particle $x$ is updated by $T_{\mu,p}(x) \rightarrow x$ with $x \sim \mu$ and $T_{\mu,p}(x) = x + \epsilon \phi^*(x)$.

\begin{prop}\label{thm:wdistance}
Let $\hat{q}_s^n$ be the empirical distribution of particles $\{x^{\ell, s} \}_{l=1}^n$ 
at the $s$-th iteration of the dynamics of our approach. 
Assume that $g(x,x^\prime) := \stein_p \odot \vv k(x, x^\prime)$ is Lipschitz continuous jointly on $\X\times\X$
% with compact set $\X$ 
and
\begin{equation}
\lim_{n\to \infty} \mathcal{W}_1(\hat{q}_0^n, ~~{q}_0^\infty) \rightarrow 0,
\end{equation}
then
\begin{equation}
\lim_{n\to \infty} \mathcal{W}_1(\hat{q}_s^n, ~~{q}_s^\infty) \rightarrow 0,
\end{equation}
at any finite iteration $s$.
% here $q_s^\infty$ is obtained by applying map \eqref{equ:gsvgd} on $x \sim q_0^\infty$ recursively for $s$ times.
\end{prop}
% \begin{proof}
% See Appendix for the derivation.
% \end{proof}

% From the above analysis we can see that as particles increase at certain iteration, the distribution converges. 
% Further it can be shown that as iteration increases, 
% Now it remains to show that limit
% distributions exactly converge to our target distribution as the number of iteration increases. 
% We then show the iterative transformations in \eqref{equ:gsvgd}
% of our algorithm monotonically decreases the KL divergence between $q_s^\infty$ and target $p$.
% From the above Proposition \label{thm:wdistance}, 
% we can see that for a nicely chosen initial distribution, 
% the weak convergence of empirical distributions at each iteration is guaranteed.

% Further, we would like to show that 
% $q_s^\infty$ converges to the target distribution $p$ as $s \rightarrow \infty$.

Further we show that the iterative transformations in \eqref{equ:gsvgd}
of our algorithm monotonically decreases the KL divergence between $q_s^\infty$ and the target distribution $p$.
% Note that the updates in original SVGD is defined in the same RKHS
% with the associated kernel defined over all coordinates.
% However, we use structured kernels $k_i$ for different coordinates $i$ specified by $\N_i$,
% which leads to a Stein discrepancy with graphical structures whose relationship with KL divergence measuring the whole coordinates is less straightforward.
% Still, we can show that under structured kernels, the decrease of KL divergence is bounded by the Stein discrepancy with graphical structures.
Moreover,
we can show that under structured kernels, the decrease of KL divergence is bounded by the Stein discrepancy with graphical structures,
indicating the fact that
Stein discrepancy $\S(\hat{q}_s^\infty~||~ p)$ tends to zero as iteration increases.

% Our conclusion is an immediate result of Theorem 4.3 in \citet{2017arXiv170407520L}.
% to make content self-contained, we detailed our results as belows. 
% In our graphical SVGD, 
% a matrix-valued positive definite kernel $\K(x,x'):= \diag(k_1,\dotsc,k_d)$ is defined, where 
% $k_i(x,x') = \exp(-\frac{||x_{\N_i} - x'_{\N_i}||^2}{h_i})$ with $\N_i$ being neighborhood of node i. 
% when we choose graphical structured kernels $k_i$ to be RBF kernels where $k_i(x,x') = \exp(-\frac{||x_{\N_i} - x'_{\N_i}||^2}{h_i})$ with $\N_i$ being neighborhood of node i, 
% we can prove that with such kernel, large sample limiting distributions converge to target distribution $p$ as iteration increases.

% \red{TODO: more novel results}
\begin{prop}\label{thm:convergence}
% \begin{enumerate}
% \item % converge as number of iteration increases
Assume that the function
$\nabla \log p$ is Lipschitz continuous with Lipschitz constant $M_1$ 
and that 
$\max\limits_{i \in [d]} 
\sup\limits_{x \in \X} k_i(x,x)
% { \E_{x \sim q_{\C_i}} k_i(x,x) }
$ is finite denoted by $M_2$. 
% $M = || \nabla \log p||_{Lip} < \infty$ 
Then for step-size $\epsilon$ smaller than $\frac{1}{M_1 M_2}$ and KL divergence $\\KL(q_0^\infty ~||~ p) < \infty$, it holds that
\begin{equation}
\KL(q_{s+1}^\infty ~||~ p) - \KL(q_s^\infty ~||~ p) \leqslant - \frac{\epsilon}{2}\S(q_s^\infty ~||~ p)^2.
\end{equation}
\end{prop}
% \begin{proof}
% % It is a direct result of Theorem 4.3 in \citet{2017arXiv170407520L}.
% See Appendix for more details.
% \end{proof}

% \red{TODO: less redundant}

Proposition \ref{thm:wdistance}
and \ref{thm:convergence} together indicate
that 
% the empirical marginal distributions of the particles weakly converge to 
% the target marginal distributions
% % , i.e. $\S(\hat{q}_s^n~||~ p) \rightarrow 0$
% as $s\rightarrow \infty, n\rightarrow \infty$.
the empirical marginal distributions $\hat{q}_{s}^n(x_{\C_i})$ weakly converge to the
target marginal distributions $p(x_{\C_i})$,
as $s\rightarrow \infty, n\rightarrow \infty$.
When these target marginal distributions define a unique distribution,
the empirical distributions have a unique limit, that is they weakly converge to the target distribution.
% Together with 
% As $s \rightarrow \infty$,
% the monotonically decreasing KL divergence indicates that 
% $\S(q_s^\infty ~||~ p) \rightarrow 0$. 
% corollary \ref{cor:sd},
% if the Stein discrepancy $\S(\hat{q}_s^n~||~ p) =0$, 
% then the target distribution $p$ is exactly recovered by $q_s^\infty$.
% By Proposition \ref{thm:wdistance} and Proposition \ref{thm:convergence}, 
% we conclude that
% as $n \rightarrow \infty$, $s \rightarrow \infty$,
% the empirical distributions $\hat{q}_{s}^n$ converge to the target distribution $p$.



% From the above Proposition \ref{thm:convergence}, 
% it can be shown that 
% the large sample limit distributions $q_s^\infty$ iteratively converge to the target distribution.
% This is because when the KL divergences between $q_s^\infty$ and $p$ converge as $s \rightarrow \infty$, 
% we have that the Stein discrepancy $\S(q_s^\infty || p) \rightarrow 0$.
% Moreover, by Corollary \ref{cor:sd},
% we obtain that if the Stein discrepancy $\S(q_s^\infty || p) =0$, then the target distribution $p$ is exactly recovered by $q_s^\infty$.

% Therefore,  as $n\rightarrow \infty, s\rightarrow \infty$.
% the convergence of our graphical SVGD is guaranteed 

% Therefore, if $\S(q_s^\infty || p) =0$, and combing with Proposition \ref{thm:wdistance}
% and Corollary \ref{cor:sd},
% then the empirical distribution $\hat{q}_s^n$
% of our graphical SVGD weakly converges to the target distribution as $n\rightarrow \infty, s\rightarrow \infty$.
% From theorem \ref{thm:convergence}, 
% we could see that when KL divergence is non-negative, 
% Stein discrepancy between $p$ and $q$ decays monotonically to zero as iteration increases,
% leading to the convergence of graphical SVGD dynamics. 
% Theorem \ref{thm:convergence} further points out that target distribution $p$ is the only limit when convergence happens. 
% Thus, convergence to target distribution is guaranteed in graphical SVGD dynamics.








==> tex/related.tex <==
\section{Related Work}
\label{sec:related_work}
% particle BP is not suitable for high-dimensional data,
% and it typically does not take the dependence strcuture
% among the variables into account.
% Introduction:
% 1. Graphical models is very useful.
% 2. Variational inference methods, especially BP methods, have been widely used.
% 3. However, most BP methods are designed for discrete variable models. Continuous (non-Gaussian) graphical models are much more difficult, and it often requires additional approximation on BP type methods. These methods include particle BP, non parametric BP, kernel BP, etc (which uses particle approximation, or kernel density approximation on typical BP methods).
% 4. The disadvantage of BP methods, however, are that they often do not leverage the gradient information of the density function. It has been shown that by leveraging the gradient information the performance can typically largely improved.
% 5. We propose a new method that leverages the gradient information as well as graphical structure information of the models. Our method is ....

% \red{TODO: more pmp and comparison with gsvgd}
% They are chosen to be baselines because like Graphical SVGD, they are also particle-based inference algorithms for graphical models and have been the most satisfying inference algorithms on continuous graphical models so far.
% PMP methods are variants of max-product (MP) belief propagation algorithms \citep{pearl1988probabilistic,aji2000generalized,wainwright2008graphical}.
% which integrate both the flexibility of sampling-based approaches and the efficiency of MP message passing \citep{trinh2009unsupervised,peng2011convex,besse2014pmbp,kothapa2011max}. Following we briefly introduce some representatives of PMP methods.
% inspired by work on particle filters and Monte Carlo methods \citep{cappe2007overview}, integrating the flexibility of sampling-based approaches and the efficiency of MP message passing \citep{trinh2009unsupervised,peng2011convex,besse2014pmbp,kothapa2011max} .
% Max-product (MP) belief propagation algorithms \citep{pearl1988probabilistic,aji2000generalized,wainwright2008graphical} as a local-message passing algorithm on graph is known to do efficient inference on graphical model with discrete distributions. For systems with continuously valued states or discrete-valued variables with very large domain, one possibility is to reduce the effective state space through random sampling \citep{arulampalam2002tutorial,koller1999general,sudderth2010nonparametric,isard2003pampas,neal2004inferring}
% The best-known example is the family of particle max-product (PMP) methods inspired by work on particle filters and Monte Carlo methods \citep{cappe2007overview}, integrating the flexibility of sampling-based approaches and the efficiency of MP message passing \citep{trinh2009unsupervised,peng2011convex,besse2014pmbp,kothapa2011max} .
% This algorithm
% essentially corresponds to a non-iterative version of the
% method described in Koller et al. (1999).
% Stochastic Proposals To allow higher-likelihood state
% configurations to be discovered, at each iteration PMP first
% creates an augmented particle set Xaug = X [ Xprop of size
% N,  > 1. New particles are drawn from proposal distributions
% Xprop  q(X). In the simplest case, Gaussian
% random walk proposals qgauss(xs) = N(xs j xs; ) sample
% perturbations of current particle locations xs (Trinh &
% McAllester, 2009; Peng et al., 2011). For some models, a
% more informative neighbor-based proposal is possible that
% samples from edge potentials qnbr(xs j xt) /  st(xs; xt)
% conditioned on a particle xt at neighboring node t 2 􀀀(s)
% (Besse et al., 2012). Specialized “bottom-up” proposals
% based on approximations of observation potentials  s(xs)
% can also be effective (Pacheco et al., 2014).
% first use stochastic proposals to augment the set of particles 
% with a candidate of hypotheses and
% then update the messages over the new particle set using the PMP
% message updates.
% Finally, we select the subset of particles which perserve the current
% message values.
% Metropolis particle Max-Product (M-PMP)
%Our particle-based update schema is 
A popular distributed inference tool for continuous graphical models is 
%mostly related to 
particle message passing (PMP) methods, 
which integrate the flexibility of sampling-based approaches and the efficiency of message-passing 
\citep{ihler2009particle, ihler2005nonparametric, sudderth2010nonparametric,  trinh2009unsupervised,peng2011convex,besse2014pmbp,kothapa2011max}.
% \citep{pearl1988probabilistic,aji2000generalized,wainwright2008graphical}.
% which integrate both the flexibility of sampling-based approaches and the 
% efficiency of message passing methods\citep{trinh2009unsupervised,peng2011convex,besse2014pmbp,kothapa2011max}. 
% Following we briefly introduce some representatives of PMP methods.
% PMP methods iteratively samples particles
% to form candidate variable assignments and find
% a MAP estimate of the resulting discrete problem with belief propagation.
% //TODOs, brief discussion about PMP methods.
% Rather than approximating the marginal expectations,
The primary differences among PMP algorithms are 
the choices of augmenting new hypotheses and selecting subset of particles
that preserve the current message values. 
The greedy PMP (G-PMP) \citep{trinh2009unsupervised,peng2011convex} chooses a single particle with highest marginal, 
which is efficient in updating particles but unable to sustain multiple modes.
% and low-effective exploration in high dimensional cases. 
% aiming to find a good non-uniform discretization for high-dimensional models. 
PatchMatch \& Top-N particle max product algorithm (T-PMP)
\citep{besse2014pmbp,pacheco2014preserving}
proposes to augment particles with samples generated from neighborhood nodes
and then retain the top $N$ particles with largest max-marginal. 
% Top-N Particle Max Product (T-PMP)\citep{pacheco2014preserving} has same particle selection rule 
% but with neighbor-based proposals appropriate for arbitrary potentials. 
Although it typically produces high-probability configurations, 
% its critically concentrated solutions harm effectiveness of particles and cause sensitivity to initialization.
% the discovered solutions of T-PMP are likely degenerate 
the simple resample-update paradigm usually lead to degeneracies.
Diverse Particle Max-Product (D-PMP) \citep{pacheco2014preserving,pacheco2015proteins} 
proposes to minimize the maximum error between max-product messages
on the augmented and reduced sets to 
% an optimization-guided stochastic selection step 
address this defect.
% by using
%distortions in MP message values,
% potentially forcing diversity into particle solutions.
Still, they suffer from sensitivity to the selection of particle resampling proposals and 
show poor performance in high-dimensional cases. %multi-modal occasion. 
% Although PMP algorithms base its inference on structure information from graphical models, 
% uncertainty in particle re-sampling and a lack of gradient information have caused their instabilities and degeneracies, 
% while the functional properties have been shown to be a significant contributor to remarkable inference performance. 
% the choice of re-sampling proposals is still unclear and critical for PMP methods.
% The Graphical SVGD we proposed leverages both graphical structure information and the gradient information from graphical distribution, which well explains why empirically it outperforms all PMP algorithms in both efficiency and sample quality. 
However, our approach has a simple form
that does not require this critical and unclear
resampling proposals selection, and also 
incorporates the key advantages of gradient-based optimization to enable 
scalable and automatic inference.
% Similarly to SVGD, our approach reduces to gradient descent
% for MAP when using only a single particle.


% owns the merits of particle-based approach, 
% and meanwhile make full use of gradient information to obtain most likely graph structure with particle diversity, 
% which well explains why it empirically outperforms the PMP algorithms in both efficiency and sample quality. 

% The Graphical SVGD we propose owns the merits of sample-based approach, and meanwhile make full use of gradient information to obtain most likely graph structure with particle diversity, which well explains why it empirically outperforms the PMP algorithms in both efficiency and sample quality. 

% Non-parametric inference with kernel embeddings of condtional
% distributions 
% The idea of using kernel trick 
The idea of using the kernel trick for inference with continuous-valued graphical models
has been discussed in a collection of recent works
% There has been a collection of recent works
% The key idea is to model each structured dat point a latent variable model,
% then embed the graphical model into feature spaces.
\citep{song2011kernel,grunewalder2012modelling,fukumizu2013kernel}.
% that uses the kernel trick for inference with continuous-valued graphical models.
% The key idea is to map conditional distributions into infinite-dimensional feature spaces using kernels, such 
% that subsequent comparisons and manipulations of these distributions are achieved via feature space operations.
The key idea is to represent the potentials as weighted sums of kernels
in a reproducing kernel Hilbert space (RKHS), which leads to simple BP updates.
The major difference, however, is that our approach
closely mimics the typical gradient descent for optimization.
This makes our approach highly flexible and scalable. 
And our algorithm can be easily combined with various state-of-the-art
techniques that have been responsible for the success of gradient optimization, including stochastic
gradient, adaptive learning rates (such as AdaGrad \citep{duchi2011adaptive}), and momentum.
% Algorithms for computing most likely configurations, or
% modes, of posterior distributions play a key role in many
% applications of probabilistic graphical models. The max-product
% variant of the belief propagation (BP) message passing
% algorithm can efficiently identify these modes for
% many discrete models (Wainwright & Jordan, 2008). However,
% the dynamic programming message updates underlying
% max-product have cost that grows quadratically with
% the number of discrete states. In domains such as computer
% vision and signal processing, we often need to estimate
% high-dimensional continuous variables for which
% exact message updates are intractable, and accurate discretization
% is infeasible.




==> tex/theory-copy.tex <==
\renewcommand{\vec}[1]{\boldsymbol{#1}}
% \newtheorem{theorem}{Theorem}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}

\newcommand{\K}{\vec{K}}
\newcommand{\vR}{\vec{R}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vvRKHS}{vector-valued RKHS }
\newcommand{\KSD}{Kernelized Stein Discrepancy }
\newcommand{\Tninv}{T_{\mu_{t+1}^n}}
\newcommand{\Tinfinv}{T_{\mu_{t+1}^\infty}}
% \newcommand{\vf}{\vec{f}}
\newcommand{\Hk}{\H_{\K}}
\newcommand{\vs}{\vec{s}}
\newcommand{\mun}{\hat{\mu}^n}
\newcommand{\muinf}{\mu^\infty}


\section{Our Approach}


% \section{Proof of the Main Results}

% Following sections are organized to firstly introduce matrix valued reproducing kernel and then \vvRKHS, allowing multi-way treatments to components.

% \subsection{\vvRKHS}

% In the following, denote by $\X$ a subset of $d-$dimensional real space $\R^d$ and $\mathcal{W}$ a Hilbert space, with $<\cdot,\cdot>_{\mathcal{W}}$ the inner product, and $\mathcal{L}(\mathcal{W})$ the Banach space of bounded linear operators on $\mathcal{W}$. A matrix valued function $\K:\X \times \X \rightarrow \mathcal{L}(\mathcal{W})$ is called a positive definite kernel if for any pair $(x,x')\in \X \times \X$, $\K(x,x')^* = \K(x,x')$ i.e. a self-adjoint operator, and
% \begin{equation}
% \sum_{i,j=1}^N <y_i,\K(x_i,x_j)y_j>_{\mathcal{W}} > 0
% \end{equation}
% for every finite set of points $\{x_i\}_{i=1}^N$ in $\X$ and $\{ y_i \}_{i=1}^N $ in $\mathcal{W}$.\\ 

% For every such $K$, there exists a unique \vvRKHS $\H_{\K}$ with reproducing kernel $\K$. Elements in $\H_{\K}$ is vector-valued functions of the form $\vf(x) = \sum_i^N \K(x_i,x)\vc_i$. Then this Hilbert space is equipped with inner product $<\cdot, \cdot>$ defined as $<\vf,\vec{g}>_{\Hk} = \sum_{i,j=1}^N <\vc_i, \K(x_i,y_j)\vec{d_i}>_{\mathcal{W}}$ between $\vf(x)$ and $\vec{g}(x) = \sum_i^N \K(y_i,x)\vec{d_i}$. The reproducing property of this Hilbert space is that for any $f$ in $\Hk$ and $\vc \in \mathcal{W}$
% \begin{equation}
% <f,\K_x \vc > = f(x)^\top \vc
% \end{equation}

% \red{A definition about $\k$}
% \red{Move stein's indentity and KSD to the background part}

% \subsection{Stein's Identity and Operator}

% \begin{mydef}
% Assume that $\X$ is a subset of $\R^d$ and $p(x)$ a continuous differentiable density whose support is $\X$. The (Stein) score function of p is defined as
% \begin{equation}
% \vec{s_p}(x) = \nabla_x \log p(x) = \frac{\nabla_x p(x)}{p(x)}
% \end{equation}
% \end{mydef}

% A funtion $\vf: \X \rightarrow \R^d$ is in the Stein class of $p$ if $\vf$ is smooth and satisfies
% \begin{equation}
% \int_{x \in \X} \nabla_x \cdot (f(x)p(x)) dx = 0
% \end{equation}

% The Stein's operator of p is a linear operator acting on the Stein class of p, defined as
% \begin{equation}
% \stein_p f = \vs_p(x)f(x) + \nabla\cdot f(x)
% \end{equation}

% \begin{lemma}(Stein's Identity)
% Assume p(x) is a smooth density supported on $\X$, then
% \begin{equation}
% \E_p[\stein_p \vf(x)] = \E_p[\vs_p(x)f(x) + \nabla\cdot f(x)] = 0
% \end{equation}
% holds for any $\vf$ in the Stein class of p.
% \end{lemma}

% \begin{lemma}
% Assume p(x) and q(x) are smooth densities supported on $\X$ and $\vf(x)$ is in the Stein class of p, we have
% \begin{equation}
% \E_q[\stein_p \vf(x)] = \E_q[(\vs_p(x) - \vs_q(x))\vf(x)^\top].
% \end{equation}
% \end{lemma}

Consider undirected graphical models of the form
$$
\log p(x) \propto \sum_{c \in \C} \psi(x_c),
$$
where $\C$ is the set of graph cliques in the graphical model.
Correspondingly, the partial derivative of $\log p$ has a nice structure as follow, with $x_i$ denoting $i^{th}$ component of $x$
$$
\partial_{x_i} \log p(x) = \sum_{ c \ni i } \partial_{x_i} \psi(x_c),
$$

One desirable property of graphical models is local Markov property: a variable $x_i$ is conditionally independent of all other nodes given its neighbors $\{ x_k \}_{k \in \N_i}$, where $\N_i$ is called the Markov blanket for a node $i$ defined as $\N_i := \cup_{i\in c}c \backslash i$.


% Recall that SVGD update is,
Recall that in SVGD update for node i, it involves all other nodes even those out of Markov blanket because of a global kernel evaluating all nodes:
$$
\begin{aligned}
x & \leftarrow x + \epsilon \phi^*(x), \\
\phi^*(x) &= \frac{1}{n} \sum_{\ell=1}^n [\nabla \log p(x^\ell)^\top k(x, x^\ell) + \nabla_{x^\ell} k(x ,x^\ell)].
\end{aligned}
$$

% motivation of improving SVGD
These redundant messages brought by independent nodes undoubtedly prevent an efficient inference performance due to its ignorance of structure information. A more wise inference algorithm leveraging both the potential of SVGD and structure information from specific graphical model is desired. We figure out a method to assign each node its update depending on its Markov blanket only, greatly improving the inference performance. 

To illustrate how these local-structure-based updates bring great improvement, consider the most extreme case when all nodes are independent from each other. Results are shown as follow

\red{TODO. fig: totally independent case}

From the above comparison we can see that, with considerations on structure information, a more effective and satisfying inference performance is obtained, meanwhile remaining both computationally tractable and simple in its updates as a remarkable feature of SVGD. 

We achieve this local structure consideration by introducing matrix-form kernel measuring Markov blankets of each node. Following we would explain in order first Stein discrepancy with the introduced matrix-form kernel, consisting foundation of our work. Then comes an elaboration of our algorithm graphical SVGD. At last we show that its convergence is theoretically guaranteed.

% We now introduce our Stein discrepancy with vector-valued RKHS.
\subsection{Stein Discrepancy in Vector-valued RKHS}
% \red{Step 1, definition about Stein discrepancy with vector-valued RKHS}
% Consider a positive define kernel $k(x, x^\prime): \X \times \X \rightarrow \R^{d\times d}$,
Denote by $\H^d = \H_1 \times \cdots \times \H_d$ the RKHS with a matrix-valued positive kernel $\k$
% consisting of function $f=[f_1, \cdots, f_d]$ with $f_i \in \H_i$,
% and 
and
inner product $\langle f, g \rangle_{\H^d} = \sum_{i=1}^d \langle f_i, g_i \rangle_{\H_i}$.
% Note that each dimension of $f$ is associated with a different RKHS with its corresponding kernel measuring neighborhoods of the $i$-th component.
Note that $f_i$'s are associated with different RKHS and corresponding kernels measuring $i^{th}$ Markov blanket.
Similarly to \citep{gorham2015measuring,oates2014control,liu2016kernelized,chwialkowski2016kernel}, 
we now define a Stein discrepancy in $\H^d$
\begin{mydef}\label{ksd_def}
Assume $\H^d=\H_1 \times \cdots \H_d$ is the \vvRKHS with matrix-valued positive definite kernel $\k$, 
and $\k$ is in the Stein class of $p$.
% Assume $\k(x, x^\prime)$ is a xxx kernel in the Stein class of $p$.
The Stein discrepancy with vector-valued RKHS
between two distributions $q$ and $p$ is defined as
\begin{equation}
\label{eq:vv_ksd}
\S_k(q,p) = \max_{f \in \H^d} \left\{ \E_{x \sim q}[ \stein_p f(x)],  ~~s.t.~~||f||_{\H^d} \le 1 \right\},
\end{equation} 
% where $f=[f_1, \cdots, f_d]^\top, f_i \in \H_i$ and 
where $\stein_p$ is the Stein's operator defined as $\stein_p f(x) = \nabla \log p(x)^\top f(x) + \nabla \cdot f(x)$.
\end{mydef}

% For a properly defined kernelized Stein discrepancy $\S_k(q,p)$, it owns a desired property that $\S(q,p)=0$ iff $q = p$. Later we would show that the matrix-valued positive definite $\K$ we adopt in our graphical svgd satisfies.
% Following we would specifically characterize the optimal function in $\Hk$ and closed form of KSD.

% \red{Introducing the reproducing property}
% $$
% \begin{aligned}
% f(x) = \langle f(\cdot), k(x, \cdot) \rangle_{\H^d} \\
% \nabla_x f(x) = \langle f(\cdot), \nabla_x k(x, \cdot) \rangle_\H
% \end{aligned}
% $$

% Let $\stein_p$ be Stein's operator of p and $\H^d$ the \vvRKHS with a matrix-valued positive definite kernel $\k$, then
% This allows us to take the expectation inside the RKHS inner product.
For simplicity, we take matrix-valued kernerl $\k$ in a diagonal form as follow, where the $i$-th diagonal entry is a positive definite kernel measuring neighborhood of $i$-th component
$$
k(x, x^\prime) = \mathrm{diag}([k_1(x, x^\prime), \cdots, k_d(x, x^\prime)]).
$$
Using the reproducing property of $\H_i$, 
% {Introducing reproducing property? appendix?}
we could shift both the expectation and Stein operator to the kernel function.
$$
\begin{aligned}
&\E_{x\sim q}[\stein_p f(x)] = \langle f, \E_{x \sim q}[\stein_p \k(x, \cdot)] \rangle_{\H^d} \\
% &= \sum_{i=1}^d \langle f, \E_{x \sim q}[ \partial_{x_i}\log p(x)\k_i(x,\cdot) + \partial_{x_i}\k_i(x,\cdot)] \rangle_{\H_i} \\
&= \sum_{i=1}^d \langle f, \E_{x \sim q}[ \stein_{p,i}k_i(x,\cdot)] \rangle_{\H_i} \\
\end{aligned}
$$
where $\stein_{p,i}f(x) = \partial_{x_i}\log p(x)f(x) + \partial_{x_i} f(x)$
is the $i^{th}$ component of $\stein_p f(x)$. Define
$$
\phi_{q,p}(\cdot) = \E_{x\sim q}[\stein_p \k(\cdot, x)],
$$
The optimization of (\ref{eq:vv_ksd}) is then framed into
$$
\max_f \langle f, \phi_{q,p} \rangle_{\H^d}, ~~s.t.~~ ||f||_{\H^d} \le 1.
$$
Similarly to \citep{liu2016kernelized,chwialkowski2016kernel},
it is direct to see that the optimal $f$ should be a normalized version of $\phi_{q,p}$.
% the maximum of $\E_{x \sim q}[\stein_p f(x)]$ when optimizing $f$
% in the unit ball of RKHS $\H^d$ related to matrix-valued kernel $\k(x, x^\prime)$.
\begin{lemma}\label{lm:optimal}
Let $\H^d$ be a vector valued RKHS related to a diagonal-valued kernel $k(x,x^\prime)$ in the 
Stein class of $p$. Denote by $\phi_{q,p}(\cdot)= \E_{x \sim q}[\stein_p k(x,\cdot))]$,
The maximum of (\ref{eq:vv_ksd}) is achieved when 
$$f=\phi_{q,p} / ||\phi_{q,p}||_{\H^d}.$$
\end{lemma}


% \begin{lemma}
% % Let $\S_k(q,p)$ be the \KSD between two distributions $q$ and $p$, 
% % and $\H^d$ be a \vvRKHS associaed with matrix-valued kernel $\k$. 
% % Then the optimal $\phi^*$ as defined in \ref{phi} maximizes \KSD. 
% Stein discrepancy with vector-valued RKHS $\S_k(q,p)$ has a closed form solution
% $$
% \S_k(q,p) = \sum_{i=1}^d \S_i(q || p), %\E_{x, x'\sim q}[ \sum_{i=1} u_p^{(i)}(x,x')]
% $$
% where 
% $$
% \begin{aligned}
% \S_i(q || p) &= s_p(x)^\top k_i(x,x^\prime)s_p(x^\prime) + s_p(x)^\top \nabla_{x^\prime} k_i(x,x^\prime)\\
% & + \nabla_{x} k_i(x,x^\prime)s_p(x^\prime)^\top + \mathrm{trace}(\nabla_{x,x^\prime} k_i(x,x^\prime)).\\
% \end{aligned}
% $$
% % where $u_p(x,x') = s_p(x')\K(x,x')s_p(x)^\top +$
% % \begin{equation}
% % \begin{split}
% % &s_p(x')[\nabla_x\cdot\K(x,x')]^\top + \nabla_{x'}\cdot\K(x,x')s_p(x)^\top\\
% % &+ \nabla_{x,x'}\cdot \K(x,x')\\
% % \end{split}
% % \end{equation}
% \end{lemma}

\begin{theorem}
Assume a positive definite matrix-valued kernel $\k=\mathrm{diag}([k_1, \cdots, k_d])$ with $k_i$ measuring neighborhood of $i^{th}$ node, then Stein discrepancy between two distribution p and q is
$$
\S_k(q, p)^2 = \sum_{i=1}^d [\S_{k_i}( q(x_i \mid x_{\neg i}), p(x_i \mid x_{\neg i}) )^2],
$$
where $\S_{k_i}$ is the Stein discrepancy defined with kernel $k_i$ measuring the difference between the conditional distributions
$q(x_i \mid x_{\neg i})$ and $p(x_i \mid x_{\neg i})$. Furthermore, a closed form solutio of $\S_{k}$ is

$$
\begin{aligned}
\S(q,p) &= \E_{x, x'\sim q}[u_p(x,x')] \\
&\text{with } u_p(x,x') = s_p(x')^\top k(x,x')s_p(x) + \\
&s_p(x')^\top\nabla_x\cdot k(x,x') + \nabla_{x'}\cdot k(x,x')s_p(x)\\
&+ \nabla_{x,x'}\cdot k(x,x')\\
\end{aligned}
$$

where $s_p(x)=\nabla \log p(x)$ is called (Stein) score function of distribution p.
\end{theorem}

\begin{proof}
By the definition of Stein discrepancy in \ref{ksd_def},
\begin{equation}
\begin{split}
&\S_{k}(q||p) = || \E_{x\sim q}[\stein_p k(x, \cdot)] ||^2 \\
&= \sum_{i=1}^d |\E_{x\sim q}[ \partial_{x_i}\log p(x) k_i(x,\cdot) + \partial_{x_i}k(x,\cdot)]|^2 \\
&= \sum_{i=1}^d |\E_{x\sim q}[ \partial_{x_i}\log p_i(x_i|x_{\neg i})k_i(x,\cdot) + \partial_{x_i}k(x,\cdot)]|^2 \\
&= \sum_{i=1}^d [\S_{k_i}( q(x_i \mid x_{\neg i}), p(x_i \mid x_{\neg i}) )^2]\\
\end{split}
\end{equation}
The closed form expression of $\S_{k_i}$ has already been given by [?], by which a closed form $\S_k$ can then be obtained.
\end{proof}

\begin{corollary}
Assume a graphical model $p$ in which the Markov blanket of node $i$ is  $\N_i$, 
and a positive definite matrix-valued kernel $\k=\mathrm{diag}([k_1(x,x^\prime), \cdots, k_d(x, x^\prime)])$,
% Let $k_i(x, x^\prime) = k_i( x_i\cup x_{N_i}, x_i^\prime \cup x_{N_i}^\prime)$, we have
it holds that
$$
\S_k (q, p)^2 = \sum_{i=1}^d [\S_{k_i} ( q(x_i \mid x_{\N_i}), p(x_i \mid x_{\N_i}))^2].
$$
\end{corollary}



\subsection{Graphical SVGD}
\red{{TODO. More discussions related to graphical models.}}
% In order to do this, we need generalize SVGD so that it uses different kernel function
% for each different coordinates, 
% $$
% \phi_i(x) = \frac{1}{n}\sum_{\ell=1}^n [ \partial_{x_i} \log p(x^\ell) K_i(x, x^\ell) + \partial_{x_i^\ell} K_i(x, x^\ell)],
% $$
% where $K_i(x^\ell, x)$ is the kernel function that is specific for coordinate $i$,

In graphical model $\log p(x) \propto \sum_{c \in \C} \psi(x_c)$ where random variables $x_i$'s depend on its Markov blanket only, we design a matrix-form kernel to effectively make use of the local Markov property. Specifically, for each positive definite real-vlaued kernel $k_i(x, x^\ell)$ in matrix-form kernel $k(x,x^\ell)$, we define it to involve only neighboring nodes of $i$ with purpose to fully capture local structure of graphical models:
$$
k_i(x, x^\prime) := k_i(x_{\N_i}, x_{\N_i}^\prime),
$$
where $\N_i$ is the Markov blanket of node $i$. As for choice of kernel, $k_i$ can be defined to be any positive definite kernel on $\N_i \times \N_i$ such as RBF kernel and Laplacian kernel. 

With a matrix-form kernel 
$
k(x, x^\prime) = \mathrm{diag}([k_1(x, x^\prime), \cdots, k_d(x, x^\prime)])
$ 
chosen, a vector valued RKHS $\H^d$ is uniquely defined by $k$, which provides an abudant funtional space to choose update $\phi$ from. Given the relation between the derivative of KL divergence and Stein discrepancy that

$$
\frac{\dno}{\dno \epsilon}   \KL(q_{[\epsilon\ff]}~||~p)  \big |_{\epsilon =0} = \E_{x\sim q}[\stein_p \ff(x)],
$$

the update velocity filed $\phi$ is chosen to maximally decrease KL divergence, which is equivalently to maximize Stein discrepancy

\begin{align}
	\phi^* & = \argmax_{\phi \in \H^d} \bigg\{  -\frac{\dno}{\dno \epsilon} \KL(q_{[\epsilon \ff]} \parallel p) \big |_{\epsilon=0} \bigg \}\\
	& = arg \max_{\phi \in \H^d} \bigg\{ \E_{x\sim q} [\stein_p \phi(x)] \bigg\},
\end{align}


By Lemma \ref{lm:optimal}, $\phi^*$ is explicitly given in a tractable form and the update can then be performed locally as follow
$$
\begin{aligned}
\phi_i(x) = & \frac{1}{n} \sum_{\ell=1} [ \partial_{x_i^\ell} \log p(x^\ell) k_i(x_{\N_i}, x_{\N_i}^\ell) \\
& + \partial_{x_i^\ell} k_i(x_{\N_i}, x_{\N_i}^\ell)]\\
\end{aligned}
$$

With updates based on exploiting interactions between neighborhoods, the inference performance on graphical models shows an exciting improvement in the joint prediction in a comprehensive manner. Our algorithm is summerized in Algorithm (\ref{alg:graphical_svgd}).
\begin{algorithm}[t] 
%\SetKwInOut{Input}{input}
\caption{Graphical SVGD} 
\label{alg:graphical_svgd}
\begin{algorithmic} 
%Observation data set $\{x_i\}_{i=1}^n$ \\%assumed to be drawn from $p(x\mid\theta)$. \\%Let $m$ be the size of mini-batch $\M$.
%\item 
%Denote the function $\mathrm{SVGD\_update}(x)$ as running stein variational gradient descent for model $p(x \mid \theta)$ \\
\STATE {\bf Input:} A target distribution with density function $p(x)$ and a set of initial particles $\{x_i^0\}_{i=1}^n$
\STATE {\bf Goal:} A set of particles $\{x_i\}_{i=1}^n$ that approximates the target distribution
\FOR{for iteration $\ell$ do} 
\STATE
$x_i^{\ell+1} \leftarrow x_i^{\ell} + \epsilon_{\ell}\phi^*(x_i^{\ell})$
\STATE
where $\epsilon_{\ell}$ is the step-size at the $\ell$-th iteration and
\STATE
$
\begin{aligned}
\phi_i(x)= & \frac{1}{n} \sum\limits_{\ell=1}[\partial_{x_i^\ell} \log p(x^\ell) k_i(x_{\N_i}, x_{\N_i}^\ell)\\
&+\partial_{x_i^\ell} k_i(x_{\N_i}, x_{\N_i}^\ell)]\\
\end{aligned}
$
\ENDFOR
\end{algorithmic} 
\end{algorithm}




\subsection{Convergence of Graphical SVGD}

Following the definition of Wasserstein distance is firstly introduced to show large sample limit of empirical distributions. Then we will show a monotonic nature in our graphical SVGD dynamics, converging to the target graphical model.

\begin{mydef}
The Kantorovich or $L_1-$Wasserstein distance between two probability measure $P_1$, $P_2$ on $\R$ wth finite mean, defined as
\begin{equation}
\mathcal{W}_1(\mu,\mu') := \inf\limits_{\gamma \in \Gamma(\mu,\mu')} \int|x-y|d\gamma(x,y)
\end{equation}
where $\Gamma(\mu,\mu') \subseteq \mathscr{P}(\R^2)$ is a family of joint distributions with marginal distribution being $\mu$ and $\mu'$ respectively.
\end{mydef}


Define a map $\Phi_p: \mu \mapsto T_{\mu,p}\mu$ characterizing graphical svgd dynamics, where $T_{\mu,p}$ is the update rule, i.e. $T_{\mu,p}(x) \rightarrow x$ with $T_{\mu,p}= x + \epsilon \phi^*(x)$.

\begin{theorem}
Let $\hat{\mu}_l^n$ be the empirical measure of $\{x_l^i \}_{i=1}^n$ at the $l$-th iteration of graphical SVGD. Assume $g(x,y):=\stein_p^x \K(x,y)$ is bounded Lipschitz jointly on $\X\times\X$ with compact set $\X$ and
\begin{equation}
\lim_{x\to \infty} \mathcal{W}_1(\mun_0,\muinf_0) \rightarrow 0,
\end{equation}
then
\begin{equation}
\lim_{x\to \infty} \mathcal{W}_1(\mun_l,\muinf_l) \rightarrow 0,
\end{equation}
at any finite iteration $l$; here $\muinf_l$ is obtained by applying $\Phi_p$ on $\muinf_0$ recursively for $l$ times as defined above.
\end{theorem}

From the above analysis we can see that as number of particles increases at certain iteration, the distribution converges. Further it can be show that as iteration increases, distributions exactly converge to our target distribution. In our graphical SVGD, a matrix-valued positive definite kernel $k(x,x'):= \diag(k_1,\dotsc,k_d)$ is defined, where 
$k_i(x,x') = \exp(-\frac{||x_{\N_i \cup i} - x'_{\N_i \cup i}||^2}{h_i})$ with $\N_i$ being neighborhood of node i. We can prove that with such kernel, distributions converges to target distribution $p$.

\begin{theorem}\label{convergence_thm}
\begin{enumerate}
\item % converge as number of iteration increases
Assume $M = || \nabla \log p||_{Lip} < \infty$ and the step-size $\epsilon$ smaller than $\frac{1}{M}$. For $KL(\mu_0^\infty || v_p) < \infty$, it holds that
\begin{equation}
KL(\mu_{l+1}^\infty || v_p) - KL(\mu_l^\infty || v_p) \leqslant - \frac{\epsilon}{2}\S_{\K}(\mu_l^\infty || v_p).
\end{equation}

\item % when converge, it is target distribution
The convergence of graphical SVGD dynamics indicates that the target distribution is exactly recovered, namely
\begin{equation}
\S_{\K}(\mu_l^\infty || v_p)=0\Leftrightarrow \mu_l^\infty = v_p.
\end{equation}
\end{enumerate}
\end{theorem}
\begin{proof}
See Appendix.
\end{proof}

From theorem \ref{convergence_thm}, we could see that since KL divergence is non-negative, KSD between $p$ and $q$ decays monotonically to zero as iteration increases, leading to the convergence of graphical SVGD dynamics. Theorem \ref{convergence_thm} further points out that target distribution $p$ is the only limit when convergenc happens. Thus, convergenct to target distribution for graphical SVGD is guaranteed.








==> tex/todos.tex <==
\section{TODOs}


